TopoClaw: A Human-Centric and Topology-Aware Agent Operating System

Large language models (LLMs) have evolved AI assistants into autonomous reasoning engines that maintain context, invoke tools, and pursue long-horizon tasks. This has spurred Agent Operating Systems (Agent OS) as kernel-like layers for lifecycle management, memory, scheduling, and access control. Yet most designs remain agent-centric, treating the OS as a single-host runtime for internal reasoning and tool use, leaving open how autonomous actions integrate with distributed, collaborative, permission-sensitive workflows. TopoClaw is an open-source, human-centric, topology-aware Agent OS modeling the user's ecosystem as two coupled structures: a physical device topology of heterogeneous surfaces and a social relationship topology of shared spaces, teams, and delegated roles. It unifies device operation, messaging, and skills around accountable cross-boundary execution, with three core contributions: (1) cross-device action placement, decoupling intent from actuation and routing distributed actions across the device cluster based on hardware affordances and user context; (2) cross-user identity attribution, treating agents as socially situated "Digital Twins" that coordinate in multi-user spaces while preserving provenance, role-aware permissions, and human accountability; (3) cross-context authority governance, pairing broad capability with distributed, context-aware policy enforcement across physical and social trust boundaries to bound proactive autonomy at the OS layer. This report presents TopoClaw as an engineering-oriented reference architecture, covering its design principles, runtime, cross-device execution, collaboration mechanisms, security model, and deployment outlook.

==> tables/tab_builtin_skills.tex <==
% Table 1: Built-in Skills
\begin{table}[H]
    \centering
    \caption{Built-in Skills Inventory}
    \label{tab:builtin_skills}
    \begin{tabular}{p{2.8cm}p{9.7cm}}
        \toprule
        \textbf{Name} & \textbf{Description} \\
        \midrule
        \multicolumn{2}{l}{\textit{Task Management}} \\
        cron & Schedule reminders and recurring tasks \\
        skill-creator & Create or update AgentSkills with scripts and assets \\
        memory & Layered workspace memory: facts, events, and grepable history \\
        personal & Build structured user memory cards through multi-layer behavioral analysis (preferences, personality archetype, core needs, behavior prediction) \\
        \midrule
        \multicolumn{2}{l}{\textit{Information Retrieval}} \\
        weather & Current weather and forecasts (no API key required) \\
        summarize & Summarize or extract text from URLs, podcasts, and local files \\
        ashare & A-share investment assistance via akshare (fundamentals, technicals, sector context) \\
        github & Interact with GitHub via \texttt{gh} CLI (issues, PRs, CI runs, \texttt{gh api}) \\
        image-collect-search & Search and retrieve high-quality images via Serper-compatible endpoint \\
        \midrule
        \multicolumn{2}{l}{\textit{Mobile Operations}} \\
        deeplink-catalog-search & Retrieve top DeepLink candidates from desktop-synced catalog \\
        set-mobile-clipboard-image & Push a base64-encoded image to the phone clipboard \\
        set-mobile-gallery-image & Push a base64-encoded image to the phone gallery \\
        send-owner-clone-message & Send a message through the owner's Digital Twin identity \\
        contacts-assistants-profile & Retrieve friends and assistant profiles from customer\_service APIs \\
        create-group-and-send-message & Create groups and send initial messages to multiple participants \\
        list-groups-and-members & List the user's groups and their members via customer\_service APIs \\
        send-group-message & Send a message to a specified group by group\_id \\
        update-group-members-and-manager & Add/remove group members and switch the group manager assistant \\
        \midrule
        \multicolumn{2}{l}{\textit{System Operations}} \\
        browser\_use & Search the web, log into websites, or extract live page content \\
        tmux & Remote control of tmux sessions \\
        \midrule
        \multicolumn{2}{l}{\textit{Protocol Extensions}} \\
        clawhub & Search and install skills from ClawHub public registry \\
        skillhub & Search and install skills from SkillHub public registry \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/tab_components.tex <==
% Table 1: Open Source Component Ecosystem
\begin{table}[htbp]
    \centering
    \caption{Open Source Component Ecosystem}
    \label{tab:components}
    \begin{tabular}{cp{9cm}}
        \toprule
        \textbf{Component} & \textbf{Description} \\
        \midrule
        TopoClaw & Core Python package, providing Agent engine, API service, multi-channel adaptation \\
        TopoDesktop & Windows desktop client, embedded TopoClaw and GroupManager, ready to use out of the box \\
        TopoMobile & Android mobile client, providing GUI automation and notification sensing capabilities \\
        customer\_service & Communication backend, responsible for message routing, device binding, and multi-device state synchronization \\
        GroupManager & Lightweight group management assistant, providing streaming dialogue capability based on pure LLM \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/tab_permissions.tex <==
% Table 2: Three-Tier File Permission System
\begin{table}[H]
    \centering
    \caption{Three-Tier File Permission System}
    \label{tab:permissions}
    \begin{tabular}{m{3cm}p{8cm}}
        \toprule
        \textbf{Tier} & \textbf{Description} \\
        \midrule
        Forbidden & The Agent cannot access these paths at all. Tool calls return permission denied directly. \\
        Read-only & The Agent can read file contents but cannot create, modify, or delete files. \\
        Editable & The Agent can freely read/write within the workspace. Write operations outside the workspace require explicit user confirmation. \\
        \bottomrule
    \end{tabular}
\end{table}


==> tables/tab_techstack.tex <==
% Table 3: Tech Stack Overview
\begin{table}[htbp]
    \centering
    \caption{Tech Stack Overview}
    \label{tab:techstack}
    \begin{tabular}{p{3cm}p{4cm}p{4.5cm}}
        \toprule
        \textbf{Layer} & \textbf{Technology} & \textbf{Rationale} \\
        \midrule
        Core Language & Python >= 3.11 & Rich ecosystem, suitable for LLM/Agent development \\
        LLM Abstraction & litellm & Unified interface, supports hot-swapping between providers \\
        Web Framework & FastAPI + uvicorn & High-performance async API, naturally aligned with LLM patterns \\
        Data Validation & Pydantic v2 & Type-safe, deeply integrated with FastAPI \\
        Real-time Comm. & WebSocket & Server-side push, streaming dialogue support \\
        Scheduled Tasks & croniter & Standard cron expression support \\
        CLI Framework & Typer & Modern CLI, more concise than Click \\
        Channel Integration & Official SDKs & Stable and reliable, version updates guaranteed \\
        \bottomrule
    \end{tabular}
\end{table}

